Spectral Temporal Graph Neural Network for Multivariate Time-series Forecasting

Multivariate time-series forecasting plays a crucial role in many real-world applications. It is a challenging problem as one needs to consider both intra-series temporal correlations and inter-series correlations simultaneously. Recently, there have been multiple works trying to capture both correlations, but most, if not all of them only capture temporal correlations in the time domain and resort to pre-defined priors as inter-series relationships. In this paper, we propose Spectral Temporal Graph Neural Network (StemGNN) to further improve the accuracy of multivariate time-series forecasting. StemGNN captures inter-series correlations and temporal dependencies \textit{jointly} in the \textit{spectral domain}. It combines Graph Fourier Transform (GFT) which models inter-series correlations and Discrete Fourier Transform (DFT) which models temporal dependencies in an end-to-end framework. After passing through GFT and DFT, the spectral representations hold clear patterns and can be predicted effectively by convolution and sequential learning modules. Moreover, StemGNN learns inter-series correlations automatically from the data without using pre-defined priors. We conduct extensive experiments on ten real-world datasets to demonstrate the effectiveness of StemGNN. Code is available at https://github.com/microsoft/StemGNN/

==> tex/analysis.tex <==
\section{Analysis}

\subsection{Traffic Forecasting}\label{section:case_traffic}

\begin{figure}[htbp]%{l}{0.5\textwidth}
    \centering
    \includegraphics[height=5.5cm,keepaspectratio]{figures/traffic.eps}
    \caption{The adjacent matrix obtained from latent correlation layer.}
    \label{adjmatrix}
\end{figure}

% \begin{wrapfigure}{l}{0.5\textwidth}
%     \centering
%     \includegraphics[height=2.8cm,keepaspectratio]{adjmatrix.eps}
%     \caption{The adjacent matrix obtained from latent correlation layer.}
%     \label{adjmatrix}
% \end{wrapfigure}

To investigate the validity of our proposed latent correlation layer, we perform a case study in the traffic forecasting scenarios. We choose 6 detectors from PEMS-BAY and show the average correlation matrix learned from the training data (the right part in Figure \ref{adjmatrix}). Each column represents a sensor in the real world.
As shown in the figure, column {\small $i$} represents the correlation strength between detector {\small $i$} and other detectors. As we can see, some columns have a higher value like column $s_1$ , and some have a smaller value like column $s_{25}$ . This indicates that some nodes are closely related to each other while others are weakly related. This is reasonable, since detector $s_1$ is located near the intersection of main roads, while detector $s_{25}$ is located on a single road, as shown in the left part of Figure~\ref{adjmatrix}. Therefore, our model not only obtains an outstanding forecasting performance, but also shows an advantage of interpretability.

\subsection{COVID-19}
\begin{table}[hb]
% \begin{table}
% \vspace{-0.4cm}  %调整图片与上文的垂直距离
	\centering
	\caption{Forecasting results (MAPE\%) on COVID-19 }\label{tab:result_on_covid19}%添加标题 设置标签
	\resizebox{\textwidth}{!}{
	\begin{tabular}{lcccccccc}	\toprule  %添加表格头部粗线
	& FC-LSTM~\cite{sutskever2014sequence} & SFM~\cite{zhang2017stock} & N-BEATS~\cite{oreshkin2019n} & TCN~\cite{bai2018empirical} & DeepState~\cite{rangapuram2018deep} & GraphWaveNet~\cite{wu2019graph} & DeelpGLO~\cite{sen2019think} & \textbf{StemGNN (ours)} \\\midrule
	7 Day & 20.3 & 19.6 & 16.5 & 18.7 & 17.3 & 18.9 & 17.1 & \textbf{15.5} \\
	14 Day & 22.9 & 21.3 & 18.5 & 23.1 & 20.4 & 24.4 & 18.9 & \textbf{17.1} \\
	28 Day & 27.4 & 22.7 & 20.4 & 26.1 & 24.5 & 25.2 & 23.1 & \textbf{19.3}\\\bottomrule
	\end{tabular}
	}
\end{table}


% \begin{table}[hb]
% % \begin{table}
% % \vspace{-0.4cm}  %调整图片与上文的垂直距离
% 	\centering
% 	\caption{Forecasting results on COVID-19 }\label{tab:result_on_covid19}%添加标题 设置标签
% 	\begin{tabular}{lccc}	\toprule  %添加表格头部粗线
%     &\multicolumn{3}{c}{MAPE(\%)}\\
% 	\cline{2-4}%\cline{7-9}\cline{11-13}
% 	&7Day &14Day &28Day\\
% 	\hline
		
% FC-LSTM~\cite{sutskever2014sequence}   &  20.3 & 22.9 & 27.4 \\
% SFM~\cite{zhang2017stock}      & 19.6 & 21.3 &   22.7 \\
% N-BEATS~\cite{oreshkin2019n}   &    16.5 &  18.5&  20.4 \\
% TCN ~\cite{bai2018empirical}      &  18.7 & 23.1 & 26.1 \\
% DeepState~\cite{rangapuram2018deep} & 17.3 &  20.4 & 24.5 \\
% GraphWaveNet~\cite{wu2019graph}& 18.9&  24.4 & 25.2 \\
% DeepGLO~\cite{sen2019think}   &17.1 &  18.9 &  23.1 \\
% \textbf{StemGNN (ours)}   & \textbf{15.5} &  \textbf{17.1 }&  \textbf{19.3}\\
% \bottomrule
% 	\end{tabular}
% \end{table}
\begin{figure}[htbp]
% \setlength{\abovecaptionskip}{0cm}   %调整图片标题与图距离
% \setlength{\belowcaptionskip}{-0.5cm}   %调整图片标题与下文距离
\centering

\subfigure[Forecasting result for the 28th day]{
\begin{minipage}[t]{0.48\linewidth}
\centering
%\includegraphics[height=5cm,width=6.7 cm]{figures/results_28_US.eps}
\includegraphics[height=5cm,width=6.7 cm]{figures/fig3.eps}
\label{analysis_fin1}
\end{minipage}%
}%
% \hspace{30px}
\subfigure[Inter-country correlations]{
\begin{minipage}[t]{0.52\linewidth}
\centering
\includegraphics[height=5cm]{figures/heatmap_top25_big.eps}
\label{analysis_fin2}
\end{minipage}%
}%
% \subfigure[Effectiveness of GFT and DFT]{
% \begin{minipage}[t]{0.33\linewidth}
% \centering
% \includegraphics[height=4cm]{figures/gft_vis_idft.eps}
% \end{minipage}%
% }%

\caption{Analysis on COVID-19}
%we visualize the {\small $U$} obtained by  the decomposition of the normalized Laplace matrix {\small $L$}, each column of {\small $U$} represents the eigenvector corresponding to the diagonal matrix of the eigenvalues, and the eigenvalues are sorted from large to small. 
%Figure (b) is a representative case between raw data and spectral domain. 
\label{analysis_fin3}
\end{figure}


To investigate the feasibility of StemGNN for real problems, we conduct additional analyses on daily number of newly confirmed COVID-19 cases. We select the time-series of 25 countries with severe COVID-19 outbreak from 1/22/2020 to 5/10/2020 (110 days). 
%Specifically, we use the first 60 days (from 1/22/2020 to 3/21/2020) for training and the rest 50 days (from 3/22/2020 to 5/10/2020) for testing. 
Specifically, we use the first 60 days for training and the rest 50 days for testing. 
In this analysis, we forecast the values of $H$ days in the future, where $H$ is set to be 7, 14 and 28 separately.
%In the testing phase, we forecast each {\small $target$} day consecutively with the historical data before {\small $target$-$H$}.
Table~\ref{tab:result_on_covid19} shows the evaluation results where we can see that StemGNN outperforms other state-of-the-art solutions in different horizons. %which respectively use historical data to forecast the number of confirmed people over the next 4 weeks.

Figure~\ref{analysis_fin1} illustrates the forecasting results of Brazil, Germany and Singapore in advance of 28 days. Specifically, we set $H=28$ and take the predicted value of the $28$th day for visualization. Each timestamp is predicted with the historical data four weeks before that timestamp. As shown in the figure, the predicted value is consistent with the ground truth. Taking Singapore as an example, after 4/14/2020, the volume has rapidly increased. StemGNN forecasts such trend successfully in advance of four weeks.
%\textcolor{red}{A further study found in appendix indicates that, thanks to spectral sequential cell in temple forecasting, StemGNN has a small time dependence, which ensures that StemGNN can timely predict the time when the data changes. The inflection point foretasted by other baselines has a significant time delay compared to StemGNN.} %In fact, the MAPE of StemGNN on Covid19  is 7.4\% higher than ohter best baselines.


% \begin{wrapfigure}{l}{0.5\textwidth}
%     \centering
%     \includegraphics[height=5.5cm]{figures/results_28_US.eps}
%     \caption{The Covid-19 results on 28 days.}
%     \label{covid28}
% \end{wrapfigure}


% \end{table}
The dependencies among different countries learned by the \textit{Latent Correlation Layer} are visualized in Figure~\ref{analysis_fin2}. Larger numbers indicate stronger correlations. We observe that the correlations captured by StemGNN model are in line with human intuition. Generally, countries adjacent to each other are highly correlated. For example, as expected, US, Canada and Mexico are highly correlated to each other, so are China, Japan and Korea.

%are not uniform across countries. This indicates that some nodes are closely related to neighboring countries while others are weakly related. This is reasonable, since countries on the same continent have higher correlations in population mobility and geographical position. Therefore, our model not only obtained the best forecasting performance, but also showed the advantage of interpretability.

% \begin{figure}
%     \centering
%     \includegraphics[height=3.5cm]{figures/fig2 (2).eps}
%     \caption{Effectiveness of GFT and DFT.}
%     \label{covid-ift-gft1}
% \end{figure}

\begin{wrapfigure}{l}{0.5\textwidth}
% \vspace{-0.4cm}  %调整图片与上文的垂直距离
% \setlength{\abovecaptionskip}{0cm}   %调整图片标题与图距离
% \setlength{\belowcaptionskip}{-0.3cm}   %调整图片标题与下文距离
    \centering
    \includegraphics[height= 4cm]{figures/fig2.eps}
    \caption{Effectiveness of GFT and DFT.}
    \label{covid-ift-gft1}
\end{wrapfigure}

We further analyze the effect of GFT and DFT in StemGNN. We choose the top two eigenvectors obtained by eigenvalue decomposition of the normalized Laplacian matrix $L$ and visualize their corresponding time-series after GFT in Figure \ref{covid-ift-gft1}. As encoded by the eigenvectors, the first time-series captures a common trend in the world and the second time-series captures a common trend from Asian countries. 
%We analyse the eigenvectors obtained by the decomposition of the normalized Laplace matrix {\small $L$}. According to \textcolor{red}{{\small $U$}}.
%we choose the component \textcolor{red}{{{\small $C0$}}} which combines the data of the main epidemic countries in the world and the component {\small $C1$} which considers the trends of Asian countries to apply the detailed analyse.  
For a clear comparison, we also visualize the ground truth of daily number of newly confirmed in the whole world and Asian countries. As shown in Figure \ref{covid-ift-gft1}, the time-series after GFT capture these two major trends obviously. Moreover, the time-series data in the spectral space becomes smoother, which increases the generalization capability and reduces the difficulty of forecasting.
%lines labeled as \textit{World} and \textit{Asian} are the ground truth for total informed number from whole world and Asian countries respectively. 
We also draw the time-series after processed by the \textit{Spectral Sequential Cell} (denoted by IDFT in Figure \ref{covid-ift-gft1}), which recognizes the data patterns in a frequency domain. Compared to the ones after GFT, the result time-series turn to be smoother and more feasible for forecasting. 

%iDFT and compare it with . We can see that those components capture these two main trends respectively, and the time-series in the graph Fourier space are relatively smooth, which also reduces the difficulty of forecasting. After spe-seq cell, the time-series in  graph Fourier space get more smooth, thus, the use of GFT and DFT can better combine the relationship matrix given by our latent correlation layer, and make the forecasting simple through feature smoothness.

%Russia and UK with high correlation are selected as cases to prove that the conversion of multivariate time-series data via GFT and DFT is effective. The upper picture in Figure~\ref{analysis_fin}(c) is the raw data of the number of infected people in the two countries (Russia, UK). We find U20, which is greatly influenced by Russial, and U16, which is greatly influenced by the UK, in the graph Fourier space according to Figure~\ref{analysis_fin}(b)and draw their shapes in space on the middle graph (U20-GFT, U16-GFT). 
%It can be seen that in the graph Fouier space, the correlation between the two components becomes high, and the data becomes smooth. Correspondingly, we analyzed the results of the corresponding components after DFT (U20-DFT, U16-DFT). In the frequency domain, the amplitude's correlation of the two components becomes higher, and the amplitude's fluctuations show regular symmetric fluctuations. Therefore, the use of GFT and DFT can better combine the relationship matrix given by our latent correlation layer, and make the forecasting simple through feature smoothness.


%To prove that the conversion of multivariate time-series data to the graph  Fourier space is effective,  we first visualize the {\small $U$} obtained by  the decomposition of the normalized Laplace matrix {\small $L$} on Figure~\ref{COVID191}(c), each column of {\small $U$} represents the eigenvector corresponding to the diagonal matrix of the eigenvalues, and the eigenvalues are sorted from large to small. We select the three eigenvectors with the largest eigenvalues ($u0-u2$). We can see that {\small $u0$}  combines the data of the main epidemic countries in the world, {\small $u1$} considers the trends of Asian countries, and {\small $u2$} considers the trends of South American countries.  According to Figure~\ref{COVID191}(b), the trends of the main epidemic countries in the world are different from the trends of Asian countries and South American countries. We also plot the time-series corresponding to the three components in the graph Fourier space on the Figure~\ref{COVID191}(b). The three components we considered capture these three main trends respectively, and the time-series in the graph Fourier space is relatively smooth~\cite{mcpherson2001birds}, which also reduces the difficulty of forecasting. Therefore, the use of GFFT can better combine the relationship matrix given by our latent correlation layer, and make the forecasting simple through feature smoothness.

==> tex/prob_def_old.tex <==
 \section{Problem Definition}

%% add an introduction, above move to chapter 1
% add GCN intro.
% pd
%preliminaries
% overview ---intro in advance
%Latent Correlations  substitute self-attention 
%overview.
%block 
%NTLST
%formula RMSE
%one step multi steps
%5/4 5.5
%has graph - one step /multi steps。 no graph。StemGNN -a -b
%StemGNNM


%\paragraph{(Spatio-temporal Graph)}
%Spatio-temporal Graph is a kind of dynamic graph structure which node attributes change with time, denoted as {\small $G=(V,E,A,X)$}, where {\small $V$} is the set of {\small $|V|= N$} vertices, {\small $E$} is the edge set, and {\small $A\in \mathbb{R}^{N\times N}$} is the adjacency matrix between two vertices in the graph. The significant difference between a spatio-temporal graph and a static graph is that its node attributes change with time, denoted as  {\small $X=\{X_1,X_2,...X_T\}\in \mathbb{R}^{T\times N\times D}$, where {\small $T$} is the step size on the time dimension and {\small $D$} is the characteristic dimension contained by each vertex.
%\paragraph{Problem Definition}

%In order to emphasize the relationship between multiple variables, we formulate the problem of multivariate time-series forecasting based on a data structure of \textit{multivariate temporal graph}, which can be formulated as {\small $\mathcal{G}=(\mathcal{V},\mathcal{E},\mathcal{X},\mathcal{W})$. {\small $\mathcal{V}=\{v_1, v_2, ..., v_N\}$} stands for the set of nodes. {\small $\mathcal{X}=\{x_{ti}\}\in \mathbb{R}^{T\times N}$} stands for the multivariate time-series input, where {\small $T$} is the total number of timestamps, {\small $N$} is the total number of univariate time-series (nodes), {\small $\bold{x}_{t}$} stands for the observed values at timestamp {\small $t$, and {\small $\bold{x}_{\cdot i} \in \mathbb{R}^{T}$} denotes the univariate time-series corresponding to node {\small $v_i$. {\small $\mathcal{E}=\{e_{ij}\}$} represents for the set of edges, where {\small $e_{ij} \in \mathcal{E}$} indicates that there is a logical dependence between two nodes {\small $v_i$} and {\small $v_j$, and {\small $w_{ij} \in \mathcal{W}$} stands for the weight associated with the edge {\small $e_{ij}$. 

In order to emphasize the relationship between multiple time-series, we formulate the problem of multivariate time-series forecasting based on a data structure of \textit{multivariate temporal graph}, which can be denoted as {\small $\mathcal{G}=(X, W)$}. {\small $X=\{x_{it}\}\in \mathbb{R}^{N\times T}$} stands for the multivariate time-series input, where {\small $N$} is the number of time-series (nodes), {\small $T$} is the number of timestamps,  {\small $\bold{x}_{t}$} stands for the observed values at timestamp {\small $ \cdot t$}, and {\small $\bold{x}_{i} \in \mathbb{R}^{T}$} denotes the univariate time-series corresponding to node {\small $i$}. {\small $W \in \mathbb{R}^{N \times N}$} is an adjacency matrix, where {\small $w_{ij} > 0$} means there is an edge between nodes {\small $i$} and {\small $j$}, and the value of {\small $w_{ij}$} denotes the strength of corresponding edge.

Given observed values of previous {\small $K$} timestamps, the task of \textit{multivariate time-series forecasting} aims to predict the node values in a multivariate temporal graph {\small $\mathcal{G}=(X, W)$} for the next {\small $H$} timestamps.
\begin{small}
\begin{equation}
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\hat{\bold{x}}_{t}, \hat{\bold{x}}_{t+1} ..., \hat{\bold{x}}_{t+H-1} = F(\bold{x}_{t-K},...,\bold{x}_{t-1};\mathcal{G};\Phi)
\end{equation}
\end{small}
where {\small $\hat{\bold{x}}_{t}, \hat{\bold{x}}_{t+1}..., \hat{\bold{x}}_{t+H-1}$} is the vector of $H$-step estimation from timestamp {\small $t$}. Given historical values {\small $\bold{x}_{t-K},...,\bold{x}_{t-1}$}, it can be inferred by model {\small $F$} with parameter {\small $\Phi$} and graph {\small $\mathcal{G}$} (input as prior or constructed automatically from data).

%\paragraph{Multivariate Temporal Graph} A multivariate temporal graph can be formulated as {\small $\mathcal{G}=(\mathcal{V},\mathcal{E},\mathcal{X},\mathcal{W})$. {\small $\mathcal{V}=\{v_1, v_2, ..., v_N\}$} stands for the set of nodes. {\small $\mathcal{X}=\{x_{ti}\}\in \mathbb{R}^{T\times N}$} stands for the multivariate time-series input, where {\small $T$} is the total number of timestamps, {\small $N$} is the total number of univariate time-series (nodes), {\small $\bold{x}_{t}$} stands for the observed values at timestamp {\small $t$, and {\small $\bold{x}_{\cdot i} \in \mathbb{R}^{T}$} denotes the univariate time-series corresponding to node {\small $v_i$. {\small $\mathcal{E}=\{e_{ij}\}$} represents for the set of edges, where {\small $e_{ij} \in \mathcal{E}$} indicates that there is a logical dependence between two nodes {\small $v_i$} and {\small $v_j$, and {\small $w_{ij} \in \mathcal{W}$} stands for the weight associated with the edge {\small $e_{ij}$. 

%In view of the particularity of multivariate time-series forecasting, we formulate the problem as a regression task based on multivariate temporal graph. 

%describe the forecast of multivariate time-series data as a time-series forecasting task based on spatio-temporal graph structure. The main purpose of spatio-temporal forecasting is to predict as much as possible the most likely attribute values of a given spatio-temporal graph node in the future based on historical observations.The formal statement is：

\iffalse
\paragraph{Multivariate Time-Series Forecasting}
Given observed values of previous {\small $K$} timestamps, the task of multivariate time-series forecasting aims to predict the values of nodes in the multivariate temporal graph {\small $\mathcal{G}=(\mathcal{V},\mathcal{E} ,\mathcal{X}, \mathcal{W})$} for the next {\small $H$} timestamps. %Mathematically, it is equivalent to solve the regression problem defined as follows:
Mathematically, it can be written as follows:
%maximizing the following log likelihood: 
%most likely attribute value sequence of the nodes contained in the multivariate temporal graph {\small $\mathcal{G}$}  in the future {\small $H$} time steps
%\textcolor{red}{regression or probability maximization?}
\begin{equation}
%\hat{X}_{t+1},...,\hat{X}_{t+H} = %\mathop{\arg\max}\limits_{X_{t+1},...,X_{t+H}}
%P(X_{t+1},...,X_{t+H}|X_{t-J+1},...,X_{t};\mathcal{G};\Phi)
 %= %\mathop{\arg\max}\limits_{X_{t+1},...,X_{t+H}}
%P(\hat{X}_{t+1},...,\hat{X}_{t+H}|X_{t-J+1},...,X_{t};\mathcal{G};\Phi)
%\min\limits_{\Phi}\sum\limits_{i=0}^{H-1}L(\bold{x}_{t+i}, \hat{\bold{x}}_{t+i}),  ~~~~~ \hat{\bold{x}}_{t+i} = F(\bold{x}_{t+i-K},...,\bold{x}_{t+i-1};\mathcal{G};\Phi)
\hat{\bold{x}}_{t}, ..., \hat{\bold{x}}_{t+H-1} = F(\bold{x}_{t-K},...,\bold{x}_{t-1};\mathcal{G};\Phi)
\end{equation}
where {\small $\hat{\bold{x}}_{t+i}, ..., \hat{\bold{x}}_{t+i+H-1}$} is the vector of H-step value estimation from timestamp {\small $t$}. Given the historical input values {\small $\bold{x}_{t+i-K},...,\bold{x}_{t+i-1}$}, it can be inferred by model {\small $F$} with parameter {\small $\Phi$} and graph {\small $\mathcal{G}$} built from the input data.
\fi

%, {\small $\hat{\bold{x}}_{t+i}$} is the corresponding vector of estimated values, which can be predicted by model {\small $F$} with parameter {\small $\Phi$} and graph structure {\small $\mathcal{G}$,. , taking {\small $\bold{x}_{t+i-K},...,\bold{x}_{t+i-1}$} as input, which is the historical multivariate time-series within a sliding window. {\small $L(.)$} denotes an arbitrary loss function, for example mean squared error in our case.

%$\hat{x}_{t+i}$} is the predicted values at timestamp {\small $t+i$, and . {\small $x_{t-i-k},...,X_{t+i-1}$} are the historical time-series values to predict {\small $\hat{x}_{t+i}$. {\small $\mathcal{G}$} is the multivariate temporal graph and {\small $\Phi$}  denotes the set of learnable parameters of the model.

%\paragraph{Auto-spatio-temporal Graph~\cite{}}



%\textcolor{red}{where {\small $|V|$} stands for the set of {\small $|V|= N$} vertices.} 
 %and {\small $A^L \in \mathbb{R}^{N\times N}$} describes the adjacency matrix between two vertices in the graph. 
   %Since most of the spatio-temporal data in real world doesn't change correlation for a relatively-shot time period, it is reasonable to suppose that {\small $G^L$} is dynamic along the time axis at set intervals, which also denoted as {\small $G^L(t^{'})$.

%\textcolor{red}{Auto-?, What is L? Dynamic graph? Adjacency matrix should be associated with weights? why use t'?}

%\paragraph{Fourier Transform~\cite{ozaktas2001fractional}}


% \begin{equation}
% \left\{
% \begin{aligned}
% \mathcal{F}(x)=\hat{x} =U^T x, \\
% %\hat{x}=\mathcal{F}(x), \\
% \mathcal{F}^{-1}(\hat{x}) = U\hat{x}
% \end{aligned}
% \right.
% \end{equation}


%\paragraph{Spectral Graph Convolution~\cite{}}
%\textcolor{red}{check the name}


==> tex/stemgnn_block.tex <==
\subsection{StemGNN Block}
The StemGNN Layer is constructed by stacking \emph{StemGNN blocks} with skip connections. A \emph{StemGNN block} is designed by plugging a Sepctral Sequential (Spe-Seq) Cell into a Spectral Graph Convolution module. In this section, we first introduce the motivation and the achitecture of the StemGNN block, and then briefly describe the Spe-Seq cell and the Spectral Graph Convolution module.

\textbf{StemGNN Block} Spectral Graph Convolution has been widely used in time-series forecasting task due to its extraordinary capability of learning latent representations of multiple time-series in the spectral domain. The key component is applying Graph Fourier Transform (GFT) to capture inter-series relationship. It is worth noting that the output of GFT is also multivariate time-series and GFT does not learn intra-series relationship explicitly. Therefore, we can utilize Discrete Fourier Transform (DFT) to learn the representations of the input time-series on the trigonometric basis in the frequency domain, which can capture the repeated patterns implicit in the periodic data or the autocorrelation features among different non-periodic timeseries. Motivated by this, we apply the Spe-Seq Cell on the output of GFT to learn temporal patterns in the frequency domain. Then the output of the Spe-Seq Cell is processed by rest components of the Spectral Graph Convolution.

Our model can also be applied to data with multiple channels. We apply GFT and Spe-Seq Cell on each individual channel $X_i$ of input data and sum the result after graph convolution with kernel $\Theta_{\cdot j}$. Then IGFT is applied on the sum to obtain the $j$th channel $Z_j$ of the output, which can be written as follows,
\begin{small}
\begin{equation}
Z_j=\mathcal{GF}^{-1}\left(\sum_ig_\Theta_{ij}(\Lambda_i)\mathcal{S}(\mathcal{GF}(X_i))\right).
\end{equation}
\end{small}
Here $\mathcal{GF}$, $\mathcal{GF}^{-1}$, and $\mathcal{S}$ denote GFT, IGFT, and Spe-Seq Cell respectively, $\Theta_{ij}$ is the graph convolution kernel for the $i$th input and the $j$th output, and $\Lambda_i$ is the eigenvalues of $X_i$. After that we concatenate $Z_j$ to obtain the final result $Z$.

We use two modules to generate predicted values. We use learnable parameters to represent basis vectors $V$ and a fully-connected layer to generate basis expansion coefficients $\theta$. Then the output $\hat{Y}=V\theta$. We have two branches of this setting in the StemGNN block, one to forecast future values, namely forecasting branch, and the other to estimate history values, namely backcasting branch. The backcasting branch helps regulate the functional space for the block to approximate signals.

Furthermore, we employ residual connections similar to \cite{oreshkin2019n} to stack multiple StemGNN blocks to build deeper models. In our case, we use two StemGNN blocks. The second block tries to approximate the residual between the groundtruth values and the approximated values from the first block. The outputs from both blocks are concatenated and passed to a GLU and fully-connected layers to generate the final predictions.

\textbf{Spectral Sequential Cell (Spe-Seq Cell)}
%It is shown in the top left part of Figure \ref{network}.
Spe-Seq Cell aims to decompose each individual time-series after GFT into frequency basis and learn feature representations on them. It  has four components in order: Discrete Fourier Transform (DFT, {\small $\mathcal{F}$}), 1D convolution, GLU and inverse Discrete Fourier Transform (IDFT, {\small $\mathcal{F}^{-1}$}), where DFT and IDFT transforms data between temporal domain and frequency domain, and 1D convolution and GLU learn feature representations in the frequency domain. Specifically, the output of DFT has real part {\small $(\hat{x}_u^r)$} and imaginary part {\small $(\hat{x}_u^i)$}, and they are processed with the same operators but different parameters in parallel. The operations can be writtent as
\begin{small}
\setlength\abovedisplayskip{3pt}
\setlength\belowdisplayskip{3pt}
\begin{align}
\label{y_N}
 %&M^{r}(y_u^{r}) = \Gamma^{r}\theta_\tau^{r}(y_u^{r}) = Y_1^{r} \odot \sigma^{r}(Y_2^{r})\\
%&M^{r}(y_u^{r}) = GLU(\theta_\tau^{r}(y_u^{r}),\theta_\tau^{r}(y_u^{r})) = \theta_\tau^{r}(y_u^{r}) \odot \sigma^{i}(\theta_\tau^{r}(y_u^{r})) \\
M^{*}(\hat{x}_u^{*}) = \text{GLU}(\theta_\tau^{*}(\hat{x}_u^{*}),\theta_\tau^{*}(\hat{x}_u^{*})) = \theta_\tau^{*}(\hat{x}_u^{*}) \odot \sigma^{*}(\theta_\tau^{*}(\hat{x}_u^{*})), *\in \{r, i\}
%&M^{i}(y_u^{i}) = GLU(\theta_\tau^{i}(y_u^{i}),\theta_\tau^{i}(y_u^{i})) = \theta_\tau^{i}(y_u^{i}) \odot \sigma^{i}(\theta_\tau^{i}(y_u^{i})) \\
%& M^{i}(y_u^{i}) = \Gamma^{i}{\theta_\tau^{i}}(y_u^{i}) = Y_1^{i} \odot \sigma^{i}(Y_2^{i})\\
%&\hat{x}_t =\mathcal{F}^{-1}(M(y_u))=\sum\limits_{t=0}^{N}M({y}_u) e^{\frac{i2\pi ut}{N+1}}, t=0,1,…,N-1
\end{align}
\end{small}
and the result $s$ can be obtained by
\begin{small}
\begin{equation}
s=M^{r}(\hat{x}_u^{r})+i M^{i}(\hat{x}_u^{i})
\end{equation}
\end{small}
where {\small $\theta_\tau^* $} is the convolution kernel with the size of 3 in our experiments, {\small $\odot$} is the the Hadamard product and nonlinear sigmoid gate {\small $\sigma^*$} determines how much information in the current input is closely related to the periodic pattern. Finally, IDFT is applied on the output $s$.

\textbf{Spectral Graph Convolution}
Spectral Graph Convolution~\cite{kipf2016semi} is composed of three steps. (1) The multivariate time-series input is projected to the spectral domain by GFT. (2) The spectral representation is filtered by a graph convolution operator with learnable kernels. (3)  Inverse Graph Fourier Transform (IGFT) is applied for the spectral representation to generate final output.

\textit{Graph Fourier Transform (GFT)}~\cite{defferrard2016convolutional} is a basic operator for Sepctural Graph Convolution. It projects the input graph to an orthonormal space where the bases are constructed by eigenvectors of the normalized graph Laplacian. The normalized graph Laplacian~\cite{ando2007learning} can be computed as: {\small $L = I_N - D^{-\frac{1}{2}}WD^{-\frac{1}{2}}$}, where {\small $I_N \in \mathbb{R}^{N\times N}$} is the identity matrix and {\small $D$} is the diagonal degree matrix with {\small $D_{ii}=\sum_j{W}_{ij}$}.  Then, we perform eigenvalue decomposition on the Laplacian matrix, forming {\small $L = U\Lambda U^T$}, where {\small $U \in \mathbb{R}^{N\times N}$} is the matrix of eigenvectors and {\small $\Lambda$} is a diagonal matrix of eigenvalues. Given multivariate time-series {\small $X \in \mathbb{R}^{N \times T}$},  the operators of GFT and IGFT are defined as {\small $\mathcal{GF}(X) = U^TX  = \hat{X}$} and {\small $\mathcal{GF}^{-1}(\hat{X}) = U\hat{X}$} respectively. The graph convolution operator is implemented as a function $g_{\Theta}(\Lambda)$ of eigenvalues $\Lambda$ with parameter $\Theta$.

==> tex/stemgnn_old.tex <==
\subsection{StemGNN Layer}

%\textbf{StemGNN Block} \quad 

As visualized in the top of Figure \ref{network}, a StemGNN block is designed by a fusion of  \textit{Spectral Sequential (Spe-Seq) Cell} and \textit{Spectral Graph Convolution}.  The \textit{Spe-Seq Cell} learns representations of the time-series on the trigonometric basis in frequency domain, which can capture the repeated patterns implicit in the periodic data or the autocorrelation characteristics among different features for the non-periodic data.  Frequency domain analysis does not depend on periodicity, so \textit{Spe-Seq Cell} is a more general algorithm. In addition, we can effectively analyze the components of the signals by combining frequency information. We combine the \textit{Spe-Seq Cell} and \textit{Spectral Graph Convolution} at Graph Fourier domain to utilize  the temporal patterns and the multivarite dependencies \textit{jointly}. We first introduce the basic of this two modules separately, and then we make a detailed look at StemGNN block.

%$\bigodot$} is the element-wise Hadamard product. 
%To simplify the description, let's call the filter {\small $g_\theta=diag(U^T g)$}  
%\textbf{Graph Fourier Transform~\cite{defferrard2016convolutional}}\quad

%\textcolor{red}{We} transform the convolution operation of the graph to the spectral domain with graph Fourier transforms, named as \textcolor{red}{spectral graph convolution}. We introduce the graph convolution operator {\small $"* \mathcal{G} "$} from the perspective of graph signal processing. In spectral domain, we use the auto-spatio-temporal graph {\small $G^L(t^{'})$} and the normalized graph Laplacian {\small $L$} to calculate the Fourier basis {\small $U\in \mathbb{R}^{N\times N}$:
%where {\small $I_N \in \mathbb{R}^{N\times N}$} is an identity matrix, {\small $D$} is the diagonal degree matrix with {\small $D_{ii}=\sum_j{W}_{ij}$}  {\small $U \in \mathbb{R}^{N\times N}$} is the matrix of eigenvectors, {\small $\Lambda$} is the diagonal matrix of eigenvalues. 
%$U$} forms an orthogonal space with {\small $U^T$: {\small $U^T U=I$} 
%We treat the input data {\small $x\in \mathbb{R}^N$as a graph signal, and each of its one-dimensional components represents the property value of a node in the graph. 


%\begin{equation}
%\left\{\begin{array}{l}
%\mathcal{GF}(X) = U^TX  = \hat{X}, \\
% %\hat{x}=\mathcal{F}(x), \\
% \mathcal{GF}^{-1}(\hat{X}) = U\hat{X}
%\end{array}\right.
%\end{equation}

\textbf{Spectral Sequential Cell} \quad
%It is shown in the top left part of Figure \ref{network}.
Multiple time-series after graph Fourier transform are orthogonal with each other and become more feasible to be predicted by sequential models.    As shown in Figure \ref{network}, a \textit{Spe-Seq Cell} can be applied to each univariate time-series separately by conducting four operators in order: (1) Discrete Fourier Transform (DFT, {\small $\mathcal{F}$}), (2) 1D convolution, (3) GLU and (4) Inverse Discrete Fourier Transform (IDFT, {\small $\mathcal{F}^{-1}$}). 
 %\textcolor{red}{Frequency domain analysis does not depend on periodicity, so Spe-Seq Cell is a more general algorithm. In addition, we can effectively analyze the components of the signals by combining frequency information. 
 %\textit{Spectral Sequential Cell} is proved in the appendix can complete the forecasting task alone, here we use this cell to learn the embedding vector of the time-series.}
% Spe-seq cell utilize the idea of modeling the time series with the linear combination of sine and cosine to do analysis in frequency domain, which  has two main advantages: for periodic data, spe-seq cell can model the period or rhythm implicit in the data; for non-periodic data, spe-seq cell can learn autocorrelation characteristics between different features.
Suppose the input time-series is {\small $\{x_t~|~ t = 0, 1, ..., N-1\}$},  firstly, we use this \textit{Spe-Seq Cell} to learn the embedding vector of the time-series and the output of DFT  is given by: {\small $\hat{x}_u=\hat{x}_u^{r} + i\hat{x}_u^{i}= \mathcal{F}(x_t)$}.
% \begin{small}
% \begin{equation}
% \setlength\abovedisplayskip{0pt}
% \setlength\belowdisplayskip{0pt}
% \label{DFT}
%   y_u=y_u^{r} + iy_u^{i}= \mathcal{F}(x_t)=\frac{1}{N}\sum\limits_{t=0}^{N-1} x_t e^{\frac{-i2\pi ut}{N}}, u=0,1,…,N-1
% \end{equation}
% \end{small}

Then we use 1D convolution and GLU to capture the features in the frequency domain. Note that the output of DFT has real part {\small $(\hat{x}_u^r)$} and imaginary part {\small $(\hat{x}_u^i)$}, thus we deal with the two parts separately which means that they have the same operation but different parameters. {\small $M^*$} denotes the module composed of 1D convolution and GLU applied separately to real and imaginary parts.  Given the input  $\small \hat{x}_u$, we define those operations as:
\begin{small}
\setlength\abovedisplayskip{3pt}
\setlength\belowdisplayskip{3pt}
\begin{align}
\label{y_N}
 %&M^{r}(y_u^{r}) = \Gamma^{r}\theta_\tau^{r}(y_u^{r}) = Y_1^{r} \odot \sigma^{r}(Y_2^{r})\\
%&M^{r}(y_u^{r}) = GLU(\theta_\tau^{r}(y_u^{r}),\theta_\tau^{r}(y_u^{r})) = \theta_\tau^{r}(y_u^{r}) \odot \sigma^{i}(\theta_\tau^{r}(y_u^{r})) \\
&M^{*}(\hat{x}_u^{*}) = \text{GLU}(\theta_\tau^{*}(\hat{x}_u^{*}),\theta_\tau^{*}(\hat{x}_u^{*})) = \theta_\tau^{*}(\hat{x}_u^{*}) \odot \sigma^{*}(\theta_\tau^{*}(\hat{x}_u^{*})), *\in \{r, i\} \\
%&M^{i}(y_u^{i}) = GLU(\theta_\tau^{i}(y_u^{i}),\theta_\tau^{i}(y_u^{i})) = \theta_\tau^{i}(y_u^{i}) \odot \sigma^{i}(\theta_\tau^{i}(y_u^{i})) \\
%& M^{i}(y_u^{i}) = \Gamma^{i}{\theta_\tau^{i}}(y_u^{i}) = Y_1^{i} \odot \sigma^{i}(Y_2^{i})\\
&M(\hat{x}_u)=M^{r}(\hat{x}_u^{r})+i M^{i}(\hat{x}_u^{i})
%&\hat{x}_t =\mathcal{F}^{-1}(M(y_u))=\sum\limits_{t=0}^{N}M({y}_u) e^{\frac{i2\pi ut}{N+1}}, t=0,1,…,N-1
\end{align}
\end{small}
Where  {\small $\theta_\tau^* $} is the convolution kernel with the size of 3 in our experiments, {\small $\odot$} is the the Hadamard product and nonlinear sigmoid gate {\small $\sigma^*$}  determines how much information in the current input is closely related to the periodic pattern. Before we apply more operations, we use the inverse transformation of the DFT with {\small $x'_t = \mathcal{F}^{-1}(M(\hat{x}_u))$}. %the following proposition:
% \begin{small}
% \setlength\abovedisplayskip{0pt}
% \setlength\belowdisplayskip{0pt}
% \begin{equation}
% \hat{x}_t = \mathcal{F}^{-1}(M(y_u)) = \sum\limits_{t=0}^{N}M({y}_u) e^{\frac{i2\pi ut}{N+1}}, t=0,1,…,N-1
% \end{equation}
% \end{small}


  %Spe-Seq Cell itself can complete the forecasting task. We use it to learn the embedding vector of the time-series .
 %\textit{Spectral Sequential Cell} is proved in the appendix can complete the forecasting task alone, here we use this cell to learn the embedding vector of the time-series.

\textbf{Spectral Graph Convolution} \quad 
A Spectral Graph Convolution~\cite{kipf2016semi} is composed of three steps. (1) The multivariate time-series input is projected to the spectral domain by GFT. (2) The spectral representation is filtered by a graph convolution operator with learnable kernels. (3) Inverse Graph Fourier Transform (IGFT) is applied for the spectral representation to generate final output.

\textit{Graph Fourier Transform (GFT)}~\cite{defferrard2016convolutional} is a basic operator for Sepctural Graph Convolution. It projects the input graph to an orthonormal space where the bases are constructed by eigenvectors of the normalized graph Laplacian. %Assume there is a multivariate temporal graph {\small $\mathcal{G}$} in the spectral domain, where {\small $N$} is the number of nodes in the graph. The normalized graph Laplacian {\small $L$} can be calculated and used to derive the Fourier basis {\small $U$} through eigenvalue decomposition:
The normalized graph Laplacian~\cite{ando2007learning} can be computed as: {\small $L = I_N - D^{-\frac{1}{2}}WD^{-\frac{1}{2}}$}, where {\small $I_N \in \mathbb{R}^{N\times N}$} is the identity matrix and {\small $D$} is the diagonal degree matrix with {\small $D_{ii}=\sum_j{W}_{ij}$}.  Then, we perform eigenvalue decomposition on the Laplacian matrix, forming {\small $L = U\Lambda U^T$}, where {\small $U \in \mathbb{R}^{N\times N}$} is the matrix of eigenvectors and {\small $\Lambda$} is a diagonal matrix of eigenvalues. Given multivariate time-series {\small $X \in \mathbb{R}^{N \times T}$},  the operators of GFT and IGFT are defined as {\small $\mathcal{GF}(X) = U^TX  = \hat{X}$} and {\small $\mathcal{GF}^{-1}(\hat{X}) = U\hat{X}$} respectively.
%As defined above, a Graph Fourier Transform operation projects the multivariate time-series input into spectral  representation {\small $\hat{X}$} constituted by the eigenvector {\small $U$} of the Laplacian matrix {\small $L$}  
%Each element in the transformed graph signal {\small $\hat{x}$} is the corresponding coordinate in the projection space. 
%In the spectral space, the representation {\small $\hat{X}$} is filtered by a graph convolution operation {\small $g_\theta$} with kernel {\small $\theta \in \mathbb{R}^N$}  which is named as spectral graph convolution: 
% \begin{equation}
% y=g_\theta*\mathcal{G}x =U g_\theta U^T x = g_\theta(L)x=g_\theta(U\Lambda U^T )x=Ug_\theta(\Lambda)U^T x
% \end{equation}
%\begin{equation}
%y=g_\theta*\mathcal{G}x = g_\theta(L)x=g_\theta(U\Lambda U^T )x=Ug_\theta(\Lambda)U^T x=\mathcal{F}^{-1}(g_\theta(\Lambda)\mathcal{F}(x))
%GraphConv(X, \theta) = Ug_\theta(\Lambda)U^\top X=\mathcal{GF}^{-1}(g_\theta(\Lambda)\mathcal{GF}(X))
%\end{equation}
%We represent the relationship between the original signal and the transformed signal as {\small $x=\sum _i \hat{x}_i u_i$}  which is the same as the inverse Fourier transform. Therefore, the operation of input signal {\small $x$} and filter {\small $g\in \mathbb{R}^N$} in the frequency domain can be defined as:
% \begin{equation}
% g_\theta*\mathcal{G}x = \mathcal{F}^{-1}(\mathcal{F}(x)\bigodot\mathcal{F}(g_\theta)) = U(U^T x\bigodot U^T g_\theta) 
% \end{equation}
%where {\small $*\mathcal{G}$} represents the convolution operator in the graph signal.
%\paragraph{3D Spectral Graph Convolution}

For a general case with multiple channels, we denote the input by {\small $X \in \mathbb{R}^{C_{in} \times N\times T}$}  where {\small $C_{in}$} is the number of input channels. Let {\small $g_\Theta$} be the graph convolution operator with kernel {\small $\Theta \in \mathbb{R}^{C_{in} \times C_{out} \times N}$}  where {\small $C_{out}$} is the number of output channels, {\small $\Theta_{ij} \in \mathbb{R}^{N}$} denotes the kernel for the {\small $i^{th}$} input and the {\small $j^{th}$} output channel. Then, a spectral graph convolution operator can be defined as:
%For multivariate temporal graph {\small $\mathcal{G}$} in specified time windows, the input can be considered to be 3D. We extend the convolution operator {\small $*\mathcal{G}$} defined in the graph signal graph  {\small $x\in \mathbb{R}^N$}  to the 3D graph signals {\small $X\in \mathbb{R}^{N\times C_i \times M}$}  containing {\small $N$} nodes, {\small $M$} time-steps and {\small $C_i$} channels. The graph convolution operator on 3D graph signals is denoted as {\small $"g_\Theta *\mathcal{G}"$}   the 3D spectral graph convolution can be defined as follows:
\begin{small}
\begin{equation}
\setlength\abovedisplayskip{0pt}
\setlength\belowdisplayskip{0pt}
Z_j = \text{GraphConv}(X, \Theta) = \mathcal{GF}^{-1}(\sum\limits_{i=1}^{C_i}g_\Theta_{ij}(\Lambda_{i}) \mathcal{GF}(X_i)) %,1\leq k \leq C_o
\end{equation}
\end{small}
%where {\small $X_i$} and {\small $U_i$} are the input representation and eigenvectors of the {\small $i^{th}$} input channel respectively. 
where  {\small $\Lambda \in \mathbb{R}^{C_{in} \times N \times N}$} is the matrix of eigenvalues and {\small $\Lambda_i \in \mathbb{R}^{N \times N}$} is a diagonal matrix containing the eigenvalues for the {\small $i^{th}$} input channel. {\small $Z_j \in \mathbb{R}^{N \times T}$} is the output in the {\small $j^{th}$} channel after IGFT, and {\small $ Z = Z_1 \oplus Z_2  ... \oplus Z_{C_{out}} \in \mathbb{R}^{C_{out} \times N \times T}$} is the final output with concatenated channels. 

%As Figure\textcolor{red}{( haven't started painting) }shows, 

%\paragraph{Spectral Sequences Forecasting} One of the most innovative part of StemGNN is that the sequential forecasting algorithm can be fully conduced in the spectral domain for a graph. Previous models for spatio-temporal forecasting~\cite{yu2017spatio,wu2019graph} are mainly based on a combination of GCN and RNN layers. It is unreasonable to stack many GCN layers in a sequence as each GCN layer requests a round of Graph Fourier Transform and inverse Graph Fourier Transformation. Moreover, the time-series along each dimension after Graph Fourier Transform are orthogonal with each other, which becomes more easier to be modeled by recurrent neural networks.  A \textcolor{red}{\textit{Spectral Sequential Cell} }is shown in the top left part of Figure \ref{network}, which is applied to the univariate time-series corresponding to each dimension after Graph Fourier Transform separately. 

%The proposition above shows the equivalence of forecasting on temporal sequences and forecasting in the frequency domain. Frequency domain analysis does not depend on periodicity, so Spe-Seq Algo is a more general algorithm. In addition, we can effectively analyze the components of the signals by combining frequency information. Spe-Seq Algo itself can complete the forecasting task. We use it to forecast the time-series data on temporal sequences.


\iffalse
\textbf{Spectral Sequential Cell} \quad
%It is shown in the top left part of Figure \ref{network}.
Multiple time-series after graph Fourier transform are orthogonal with each other and become more feasible to be predicted by sequential models. As shown in Figure \ref{network}, a \textit{Spectral Sequential (Spe-Seq) Cell} can be applied to each univariate time-series separately by conducting four operators in order: (1) Discrete Fourier Transform (DFT), (2) 1D convolution, (3) GLU, and (4) inverse DFT (IDFT). Suppose the input time-series is {\small $\{x_t~|~ t = 0, 1, ..., N-1\}$} and we want to predict the value of {\small $x_N$}  First, the output of DFT is given by: 
\begin{small}
\begin{equation}
\setlength\abovedisplayskip{0pt}
\setlength\belowdisplayskip{0pt}
\label{DFT}
   y_u=\frac{1}{N}\sum\limits_{t=0}^{N-1} x_t e^{\frac{-i2\pi ut}{N}}, u=0,1,…,N-1
\end{equation}
\end{small}
Then, if {\small $x_N$} is added to the original sequence, the corresponding sequence in the frequency domain will have {\small $N+1$} points, denoted as {\small $\{\hat{y}_0, \hat{y}_1, ..., \hat{y}_{N}\}$}. We can predict the value of {\small $\hat{y}_N$} by {\small $M(y_0, y_1, ..., y_{N-1})$}  where {\small $M$} denotes the module composed of 1D convolution and GLU.
{\small $M$} can be described as:
%\begin{equation}
  {\small $M(y) = \Gamma{*_\tau}(y_u) = Y_1 \bigodot\sigma(Y_2),$}
%\end{equation}
where {\small $*_\tau $} is the convolution kernel, {\small $\Gamma$} represents the GLU opreation, {\small $Y_1, Y_2$} is the 1D convolution map of input {\small $y)u$},  {\small $\bigodot$} is the the Hadamard product and nonlinear sigmoid gate {\small $\sigma$}  controls which information can pass through.

%\textcolor{red}{equations may needed}
%Then, {\small $\{\hat{y}_0, \hat{y}_1, ..., \hat{y}_{N-1}\}$} can be calculated based on {\small $x_t$}  {\small $y_u$} and {\small $\hat{y}_N$:
%\begin{equation}
%\label{adjustment}
%\hat{y}_u = y_u - \sum_{t=0}^{N-1}x_t\frac{e^{-\frac{i2\pi ut}{N+1}}}{N+1} + (\hat{y}_N - B)e^{\frac{i2\pi (N-u)N}{N+1}}, u=0,1,2,...,N-1
%\end{equation}
%where {\small $A=y_u - \sum_{t=0}^{N-1}x_t\frac{e^{-\frac{i2\pi ut}{N+1}}}{N+1}, B=\frac{1}{N+1}\sum_{t=0}^{N-1}x_te^{-\frac{i2\pi Nt}{N+1}}$} 

Next, given historical values and estimated value of {\small $\hat{y}_N$}  we can calculate the estimated values in the frequency domain by IDFT:
% \begin{small}
% \setlength\abovedisplayskip{0pt}
% \setlength\belowdisplayskip{0pt}
% \begin{equation}
%      \hat{x}_N = \hat{y}_N(N+1)e^{\frac{i2\pi N^2}{N+1}} - \sum\limits_{t=0}^{N-1}x_t e^{\frac{i2\pi N(N-t)}{N+1}} 
% \end{equation}
% \end{small}
% \begin{small}
% \setlength\abovedisplayskip{0pt}
% \setlength\belowdisplayskip{0pt}
% \begin{equation}
%      \hat{y}_u = y_u + \sum_{t=0}^{N-1}x_t(\frac{e^{-\frac{i2\pi ut}{N}}}{N}-\frac{e^{-\frac{i2\pi ut}{N+1}}}{N+1}) + \frac{x_N}{N+1}e^{-\frac{i2\pi uN}{N+1}}
% \end{equation}
% \end{small}
% \begin{small}
% \setlength\abovedisplayskip{0pt}
% \setlength\belowdisplayskip{0pt}
% \begin{equation}
%      \hat{x}_t =\sum\limits_{t=0}^{N}\hat{y}_u e^{\frac{i2\pi ut}{N+1}}, t=0,1,…,N
% \end{equation}
% \end{small}

\begin{small}
\setlength\abovedisplayskip{-15pt}
\setlength\belowdisplayskip{0pt}
\begin{align}
\label{y_N}
   & \hat{x}_N = \hat{y}_N(N+1)e^{\frac{i2\pi N^2}{N+1}} - \sum\limits_{t=0}^{N-1}x_t e^{\frac{i2\pi N(N-t)}{N+1}} \\
  & \hat{y}_u = y_u + \sum_{t=0}^{N-1}x_t(\frac{e^{-\frac{i2\pi ut}{N}}}{N}-\frac{e^{-\frac{i2\pi ut}{N+1}}}{N+1}) + \frac{x_N}{N+1}e^{-\frac{i2\pi uN}{N+1}} \\
  & \hat{x}_t =\sum\limits_{t=0}^{N}\hat{y}_u e^{\frac{i2\pi ut}{N+1}}, t=0,1,…,N
\end{align}
\end{small}
Here {\small $x_0, x_1, ..., x_{N-1}$} are historical values, and {\small $\hat{x}_0, \hat{x}_1, ..., \hat{x}_N$} serve as predicted values at the time domain. Detailed derivation can be found in the appendix.
\fi

%At last, we calculate the predicted value {\small $\hat{x}_N$} in the time domain based on inverse DFT:
%\begin{equation}
%\label{inverse_DFT}
%\hat{x}_t=\sum\limits_{u=0}^{N}\hat{y}_u e^{\frac{i2\pi ut}{N}}, t=0,1,…,N
%\end{equation}

%\begin{proposition}[Spectral Sequential Cell] Assume {\small $x_0, x_1, ..., x_{N-1}$} and {\small $\hat{x}_0, \hat{x}_1..., \hat{x}_{N-1}, \hat{x}_N$} are the input and output sequences of Spectral Sequential Cell. Then, we have {\small $x_t = \hat{x}_t$} for {\small $t = 0, 1, ..., N=1$}  and {\small $\hat{x}-N$} is the predicted value at timestamp {\small $N$}  (see appendix for the proof)
%\end{proposition}

%where the formulation of DFT and inverse DFT are given in Equation (\ref{DFT}) and (\ref{IDFT}) respectively. 
%Firstly, we prove the equivalence of forecasting on temporal sequences and forecasting in the frequency domain. Without loss of generality, the 
%Discrete Fourier Transform(DFT, {\small $F$) and inverse Discrete Fourier Transform(iDFT, {\small $f$)  can be defined as follow:
%\begin{equation}
%\label{DFT}
%   F(u)=\frac{1}{N}\sum\limits_{x=0}^{N-1} f(x) e^{\frac{-i2\pi ux}{N}}, u=0,1,…,N-1
%\end{equation}
%\begin{equation}
%\label{IDFT}
%   f(x)=\sum\limits_{u=0}^{N-1}F(u) e^{\frac{i2\pi ux}{N}}, x=0,1,…,N-1
%\end{equation}
%where {\small $N$} is the number of discrete timestamps. 

\iffalse
The following proposition can be obtained:

\begin{proposition}[Spectral sequential Cell] Assuming that the next value of {\small $F(u)$} can be predicted as {\small $F'(N)$}  
other unknown variables in the time and frequency domains, including the (N+1)th discrete sample f(N) and the new DFT's result  F'(u), u=0,1,2,…,N-1  are determined by the given F' (N).
\end{proposition}

We can simply proof this proposition: Let {\small $A=\sum_{x=0}^{N-1}f(x)(\frac{e^{-\frac{i2\pi ux}{N}}}{N}-\frac{e^{-\frac{i2\pi ux}{N+1}}}{N+1}), B=\frac{1}{N+1}\sum_{x=0}^{N-1}f(x)e^{-\frac{i2\pi Nx}{N+1}}$}  which can be calculated by the known values. For {\small $u=0,1,2,...,N-1$}   the value of {\small $F'(u)-F(u)$} can be represented as {\small $A + \frac{1}{N+1}f(N)e^{-\frac{i2\pi uN}{N+1}}$}  For {\small $u=N$}  the value of {\small $F'(N)$} can be represented as {\small $B + \frac{1}{N+1}f(N)e^{-\frac{i2\pi N^2}{N+1}}$}  Given {\small $F'(N)$}  we can infer {\small $f(N)$} by {\small $f(N) = (N+1)(F'(N)-B)e^{-\frac{i2\pi N^2}{N+1}}$} and {\small $F'(u)$} by {\small $F'(u)=A+(F'(N)-B)e^{\frac{i2\pi (N-u)N}{N+1}}, u=0,1,2,...,N-1$}  Thus, the only variable needs to be predicted is {\small $F' (N)$} 
% \begin{equation}
% f(N) = (N+1)(F'(N)-B)e^{-\frac{i2\pi N^2}{N+1}}
% \end{equation}
% For {\small $u=0,1,2,...,N-1$} 
% \begin{equation}
% F'(u)=A+(F'(N)-B)e^{\frac{i2\pi (N-u)N}{N+1}}
% \end{equation}

Frequency domain analysis does not depend on periodicity, so spectral sequential forecasting is a more general algorithm. In addition, we can effectively analyze the components of the signals by combining frequency information. Spectral sequential forecasting itself can complete the forecasting task. We use it to forecast the time-series data on temporal sequences. In our work,  a DFT operation is applied to transform each univariate time-series into the frequency domain. Next, we perform 2-D convolution and GLU to capture the features of spectral sequences in sequences forecasting layer, which is shown on Figure\ref{network}.  Giving the input  {\small $F(u)$}  the forecasting operation can be described as:
%\begin{equation}
  {\small $\Gamma{*_\tau}F(u) = Y_1 \bigodot\sigma(Y_2),$
%\end{equation}
where {\small $*_\tau $} is the convolution kernel, {\small $\Gamma$} represents the GLU opreation, {\small $Y_1, Y_2$} is the 1DConv map of input {\small $F(u)$}  {\small $\bigodot$} is the the Hadamard product and nonlinear sigmoid gate {\small $\sigma()$}  controls which information can pass through. Before we apply more operators, we use the inverse transform of the DFT, IDFT cell shown on Figure\ref{network}.

\fi

%Frequency domain analysis does not depend on periodicity, so spectral sequential forecasting is a more general algorithm. In addition, we can effectively analyze the components of the signals by combining frequency information. Spectral sequential forecasting itself can complete the forecasting task. We use it to forecast the time-series data on temporal sequences. In our work,  a DFT operation is applied to transform each univariate time-series into the frequency domain. Next, we perform convolution and GLU operations on the time-series before transforming them back to time domain. 1DConv cell shown on Figure\ref{network}, followed by the gated liner units(GLU), GLU cell shown on Figure\ref{network}, to capture the features of spectral sequences. Giving the input  {\small $F(u) \in \mathbb{R}^{N\times C_{i}\times M} {\small $}  the convolution kernel {\small $\Gamma*_\tau \in \mathbb{R}^{1\times K \times (2C_o) \times C_i}$} can be represented as the mapping from the input to the output {\small $[Y_1,Y_2]\in \mathbb{R}^{N\times (M-K+1)\times (2C_o) }$}  {\small $Y_1, Y_2 \in \mathbb{R}^{N\times (M-K+1) \times C_o}$} are the input of gates in gated liner units(GLU) and we use {\small $\bigodot$} to denote the Hadamard product.  We use the nonlinear sigmoid gate {\small $\sigma(Y_2)$}  to control the rate at which the input information of {\small $Y_1$} passes through the gate, which determines how much information in the current input is closely related to the periodic pattern and dynamic transformation in the target sequence. As a result, the spectral sequences forecasting  operation can be defined as:



 % with the following proposition:

%\textcolor{red}{Make sure the difference between DFT and FFT. Correct inconsistency.}

% \begin{proposition}[Spectral sequential forecasting]
% Let {\small $f(x)=\{X_0,X_1,…,X_{N-1}\}$} be a sequence with {\small $N$} time-times, {\small $F(u)=\{U_0,U_1,…,U_{N-1}\}$}  be the input representation of Discrete Fourier Transform (DFT), {\small $\{X'_0,X'_1,…,X'_{N-1}\}$}  be the output representation of DFT, which also serves as the input of inverse DFT. {\small $X_{N}$} is the representation to be predicted and {\small $\hat{U}'_{N}$} is the predicted value. Other unknown variables in the time and frequency domains, including {\small $X'_{N}$} and {\small $\{U'_0,U'_1,…,U'_{N-1}\}$}  are determined given {\small $\hat{U}'_{N}$}  Then {\small $X_{N}$} can be calculated by {\small $\hat{F}'(u)=\{U'_0,U'_1,…,U'_{N-1},\hat{U}'_{N}\}$}  where {\small $u=\{0,1,…,N-1\}$:


% \begin{equation}
%  A=\sum\limits_{x=0}^{N-1}f(x)(\frac{e^{-\frac{i2\pi ux}{N}}}{N}-\frac{e^{-\frac{i2\pi ux}{N+1}}}{N+1})
% \end{equation}
% \begin{equation}
%  B=\frac{1}{N+1}\sum\limits_{x=0}^{N-1}f(x)e^{-\frac{i2\pi Nx}{N+1}}
% \end{equation}

% \begin{equation}
% \hat{F}'(u)=A+(\hat{U}'_{N}-B)e^{\frac{i2\pi (N-u)N}{N+1}}
% \end{equation}

% \end{proposition}

% With the input of the 3D graph signal {\small $X \in \mathbb{R}^{N\times C_{i}\times M} {\small $}  we define the  DFT operation, FFT cell shown on Figure\ref{network}, as follows:
% %$x = SX$

% %Fast Fourier Transform on each uni variate time-series separately, FFT cell shown on Figure \ref{network}. , on the {\small $K$} neighbors of each node in graph {\small $\mathcal{G}$} to obtain a sequence representation in the frequency domain. 


% \begin{equation}
%   F(u)=\frac{1}{M}\sum\limits_{i=0}^{M-1} X_i e^{\frac{-i2\pi ui}{M}} , u=0,1,…,M-1
% \end{equation}




% \begin{equation}
%   X=F^{-1}(F(u))=\sum\limits_{x=0}^{(M-K+1)}\Gamma_{*\tau}F(u) e^{\frac{i2\pi uX}{(M-K+1)}} \in  \mathbb{R}^{S\times (M-K+1) \times C_o}
% \end{equation}
% \begin{equation}
%   F^{-1}(x)=\sum\limits_{u=0}^{(M-K+1)}\Gamma{*_\tau}F(u) e^{\frac{i2\pi ux}{(M-K+1)}} \in  \mathbb{R}^{N  \times (M-K+1) \times C_o}, x=0,1,…,M-K
% \end{equation}

%\text{Spectral Residual Layer}
\textbf{StemGNN Block}\quad % - Spectral Temporal Graph Convolution}\quad 
%\subsubsection{Spectral Temporal Graph Convolution}
Based on the definition of Spectral Graph Convolution and \textit{Spectral Sequential Cell}, a StemGNN block can be formulated as a fusion of these two components, which is defined as below,
\begin{small}
\setlength\abovedisplayskip{0pt}
\setlength\belowdisplayskip{5pt}
\begin{align}
\label{equ:Z}
& Z_j=\mathcal{GF}^{-1}(\sum\limits_{i=1}^{C_i}g_\Theta_{ij} (\Lambda) \mathcal{F}^{-1}(M(\mathcal{F}(\mathcal{GF}(X))))) \nonumber\\
& Z = Z_1 \oplus Z_2 ... \oplus Z_{C_{out}} \in \mathbb{R}^{C_{out} \times N \times T}
\end{align}
\end{small}
where {\small $\mathcal{F}(\cdot)$} and {\small $\mathcal{F}^{-1}(\cdot)$} denote DFT and  IDFT respectively;
 {\small $\mathcal{GF}(\cdot)$} and {\small $\mathcal{GF}^{-1}(\cdot)$} denote GFT and IGFT respectively;
{\small $M$} denotes the modeling function in the frequency domain (1D convolution + GLU); $g_\Theta_{ij}$ denotes graph convolution with kernel $\Theta$ for the $i^{th}$ input and $j^{th}$ output channel; and {\small $Z$} is the final output representation obtained by a concatenation of individual output channels. 

Afterwards, {\small $Z$} is fed to a fully-connected layer, which generates the coefficients {\small $\theta^f \in \mathbb{R}^{B}$} for basis vector combination, where {\small $B$} is the number of basis. There are two output modules. In the forecasting module, the final output can be computed by {\small $\hat{Y} = V^f\theta^f$}, where {\small $V^f \in \mathbb{R}^{D \times B}$} contains basis vectors that are jointly learned in the networks, and {\small $D$} is the dimension of basis vectors. The backcasting module works similarly to generate the corresponding output.

%The StemGNN blocks produce basis expansion coefficients both forecast$(\theta^f)$}  and backcast$(\theta^b)$to the basis layers {\small $g^f$} and {\small $g^b$}  So the output of {\small $i$} StemGNN block  are {\small $\hat{Y}_{li} = g^f_i(\theta^f_i)$} and {\small $\hat{X}_{li} = g^b_i(\theta^b_i)$} 
%and {\small $Y=\{Y_1, Y_2, ... Y_{C_{out}}\}$} is the representation containing all output channels. 
%The above graph convolution directly processes the graph structure data, and can extract the feature attributes of node level in the target region and the spatial information in the neighborhood. In order to connect the nodes in different time steps, we combine the 3D spectral graph convolution and spectral sequences forecasting in the frequency domain, which can simultaneously extract the organizational structure and transform characteristics of multidimensional data , written as {\small $F_{SSA}$:
%we expand the graph structure data along the timeline into a auto-spatio-temporal Graph {\small $G^L(t^{'})$}  By using spectral sequences algorithm in the frequency domain, StemGNN can simultaneously extract the organizational structure of multidimensional data in spatial dimension and transform characteristics in temporal dimension, written as {\small $F_{SSA}$:
%The architecture has two remaining branches, one acting on backcast prediction branch, written as {\small $g_\theta^b$} and the other working on forecast prediction branch, written as {\small $g_\theta^f$}  Typically, the length of the input window is set to a multiple of the predicted horizon {\small $H$}   Besides, each block outputs a partial prediction that is aggregated first at the stack level. 
%\subsection{ Spectral Sequences Algorithm}
%\textbf{Residual Connection}\quad
Furthermore, the StemGNN layer can be constructed by two StemGNN blocks with a residual connection similar to \cite{oreshkin2019n}. Let {\small $X$} be the input, and {\small $\hat{X}_1$} and {\small $\hat{Y}_1$} be the backcasting and forecasting outputs from the first StemGNN block. The input to the second block will be {\small $X - \hat{X}_1$} --- the reconstruction error from the first block, and the outputs will be {\small $\hat{X}_2$} and {\small $\hat{Y}_2$}. The motivation behind is that we can force the second StemGNN block to learn residual information that is not well captured by the first block. The outputs are the concatenation of outputs from two blocks, i.e., {\small $\hat{X} = \hat{X_1} + \hat{X_2}$},   {\small $\hat{Y} = \hat{Y_1} + \hat{Y_2}$}. Finally, both of them are fed into an output layer consisting of GLU and fully-connected layers to generate final value predictions. %\textcolor{red}{final outputs: GLU and FC}. 

%The residual architecture has two StemGNN blocks, the second StemGNN block takes the residual of raw input {\small $X_{l1}$} and {\small $\hat{X}_{l1}$} as input, and the final estimation {\small $Y$} aggregate the output from two StemGNN blocks. The output of residual forecast value {\small $\hat{Y}$} can be calculated by {\small $\hat{Y}_{l1}+\hat{Y}_{l2}$} and backcast value {\small $\hat{X}$} is {\small $\hat{X}_{l1}+\hat{X}_{l2}$}  %the following equations:
%  \begin{equation}
% X_{l_i} = X_{l_{i-1}}-\hat{X}_l_{i-1} , \hat{X} = \sum\limits_{i}^{n=2} \hat{X}_i, Y = \sum\limits_{i}^{n=2} Y_i
% \end{equation}

% where {\small $X_i$} is the input of {\small $i$} StemGNN block, which {\small $X_1$} is the raw input .


%\textcolor{red}{I think we need more formulation here.}

%It takes input {\small $\mathcal{G}$} into the well-designed graph neural network and produces basis expansion coefficients both forward(forecast), {\small $\theta^f$}  and backward(backcast),$\theta^b$}  

%A standard \textit{Bilevel Residual layer} can be constructed by two StemGNN blocks sharing the same parameters {\small $g^f$} and {\small $g^b$}  The second StemGNN block takes the residual of {\small $\mathcal{X}$} and {\small $\hat{x}$} as input, and the final estimation {\small $Y$} aggregate the output from two StemGNN blocks. The operations are defined as:

%\textcolor{red}{where}

%The two StemGNN blocks have layers with shared {\small $g^f$} and {\small $g^b$}  which can supply the basis vectors to produce the partial forecast {\small $y$} and {\small $\hat{x}$}  the estimate of {\small $\mathcal{X}$}  
 
 %two outputs {\small $\hat{X}',Y$}  {\small $\hat{X}'$} is the reconstruction of {\small $\mathcal{X}$}  which is called backcast and  {\small $Y$} is the data of {\small $H$} time-steps expected to be predicted, which is called forecast. 
 %Internally, the StemGNN block can learn the graph structure and time dynamic character from the whole input.
 
 %\subsection{Loss function}
 %\paragraph{Output Layer} 
 
\iffalse
 After passing the residual StemGNN layer, we add an output layer composed of Gated Linear Unit (GLU) and Fully-Connected (FC) sub-layers.
 %as temporal convolution  operation to predict values. %\textcolor{red}{Why softmax, isn't it a regression problem?}
 %The output of temporal convolution can be used as a single-step prediction, and then the final prediction result {\small $Z \in \mathbb{R}^{N \times c}$} is obtained. 
 %The prediction value {\small $\hat{Y}$} and the backcasting values {\small $\hat{X}$} can be calculated by the final FC layer. % using linear transformation {\small $Z\omega + b$} of {\small $c$} channels, in which {\small $\omega \in \mathbb{R}^c$} is the weight vector and {\small $b$} is the bias term. \textcolor{red}{what's the purpose of this?}
%\paragraph{Loss Function}
Given historical values at timestamp {\small $t$}  \textit{i.e.}, {\small $\{X_{t-K},...,X_{t-1}\}$}  the network will output the forecasting values for the next {\small $H$} timestamps, \textit{i.e.}, {\small $\hat{Y} = \{\hat{X}_{t}, \hat{X}_{t+1}, ..., \hat{X}_{t+H-1}\}$}  and the backcasting values {\small $\hat{X} =\{\hat{X}_{t-K},...,\hat{X}_{t-1}\}$} for reconstruction. The loss function can be formulated as: 
\begin{small}
\begin{equation}
\setlength\abovedisplayskip{0pt}
\setlength\belowdisplayskip{0pt}
L(\hat{X}, X;\Delta_\theta) = \sum\limits_{t=0}^{T-H}\sum\limits_{h=0}^{H-1}||\hat{X}_{t+h} - X_{t+h}||^2 + \sum\limits_{t=K}^{T}\sum\limits_{i=1}^{K}||\hat{X}_{t-i} - \hat{X}_{t-i}||^2
\end{equation}
\end{small}
where {\small $\Delta_\theta$} denotes all parameters that can be trained in the entire network. The first term represents for forecasting loss and the second term is for backcasting. 
%$\alpha$} is a hyperparatmer to balance the contribution of two losses, which we simply set as 1 in our experiments without tuning. 
$X_{t}$} is the ground truth matrix at timestamp {\small $t$}  while {\small $\hat{X}_{t}$} is the corresponding prediction from StemGNN.

\fi

%And the backcasting outputs are used in a auto-encoder fashion to improve the data representation model. The loss function can be written as: 
%\begin{equation}
%L(X';\Delta_\theta) = \sum\limits_{i=0}^{t-1}(||X'_i - X_i||^2)
%\end{equation}

%$\{\hat{\bold{x}}_{t+i}, ..., \hat{\bold{x}}_{t+i+H-1}\}$} denotes the forecasting value of the next timestamps and {\small $\{\bold{\hat{x}}_{t+i-K},...,\bold{\hat{x}}_{t+i-1}\}$} is used for training an auto-encoder to improve the representation model.

%Given the historical input {\small $\{\bold{x}_{t+i-K},...,\bold{x}_{t+i-1}\}$}  {\small $\hat{\bold{x}}_{t+i}$} denotes the forecasting value of the next timestamp and {\small $\{\bold{\hat{x}}_{t+i-K},...,\bold{\hat{x}}_{t+i-1}\}$} is used for training a auto-encoder to improve the representation model.

%which is by design to model multivariate and temporal dependencies in the spectral domain. There are two outputs of a StemGNN block, {\small $\hat{y}_{t+1}$} and {\small $\hat{x}$}  where {\small $\hat{y}_{t+1}$} denotes the forecasting value of the next timestamp and {\small $\hat{x}$} is used for auto-regression. 

%The forecasting loss can be defined by: {\small $L(\hat{X};\Delta_\theta) = \sum\limits_{t}(||\hat{X}_{t+H} - X_{t+H}||^2)$}  where {\small $\Delta_\theta$} is all parameters that can be trained, {\small $} X_{t+H}$} is the real data at {\small $t$} time, and {\small $\hat{X}_{t+H}$} is the predicted value of the model output. The auto-regression loss can be defined by: {\small $L(X';\Delta_\theta) = \sum\limits_{i=0}^{t-1}(||X'_i - X_i||^2)$} 

%So far, the loss function of StemGNN for multivariate time-series forecasting can be expressed as:

%\begin{equation}
%\mathcal{L} = L(\hat{X};\Delta_\theta) + L(X';\Delta_\theta)
%\end{equation}


